Detecting Low-Degree Truncation

We consider the following basic, and very broad, statistical problem: Given a known high-dimensional distribution ${\cal D}$ over $\mathbb{R}^n$ and a collection of data points in $\mathbb{R}^n$, distinguish between the two possibilities that (i) the data was drawn from ${\cal D}$, versus (ii) the data was drawn from ${\cal D}|_S$, i.e. from ${\cal D}$ subject to truncation by an unknown truncation set $S \subseteq \mathbb{R}^n$. We study this problem in the setting where ${\cal D}$ is a high-dimensional i.i.d. product distribution and $S$ is an unknown degree-$d$ polynomial threshold function (one of the most well-studied types of Boolean-valued function over $\mathbb{R}^n$). Our main results are an efficient algorithm when ${\cal D}$ is a hypercontractive distribution, and a matching lower bound: $\bullet$ For any constant $d$, we give a polynomial-time algorithm which successfully distinguishes ${\cal D}$ from ${\cal D}|_S$ using $O(n^{d/2})$ samples (subject to mild technical conditions on ${\cal D}$ and $S$); $\bullet$ Even for the simplest case of ${\cal D}$ being the uniform distribution over $\{+1, -1\}^n$, we show that for any constant $d$, any distinguishing algorithm for degree-$d$ polynomial threshold functions must use $\Omega(n^{d/2})$ samples.

==> dkp-sosa-thing.tex <==
%\section{Distinguishing LTF Truncation of Log-Concave Distributions}
%\label{appendix:dkp-sosa}
%
%In the specific setting when the background distribution is the standard $n$-dimensional Gaussian distribution, De, Nadimpalli, and Servedio~\red{TODO:SODA citation} obtained a $O_\eps(\sqrt{n})$ distinguisher but with a worse $\epsilon$-dependence. \red{TODO: write this up more clearly.}
%
%
%\
%
%
%Can assume the distribution is isotropic. 

==> lb-old.tex <==
%!TEX root = hypercontractive-product-domains.tex

\section{An $\Omega(n^{d/2})$-Sample Lower Bound for Distinguishing PTFs}
\label{sec:lb}



%\rnote{Should we give the simple argument which shows that if $p=n^{d/2}/2^n$ for the $\{-1,1\}^n$ setting, we can get an $\Omega(n^{d/4})$ lower bound? Maybe it's worth doing this (in an appendix) as a sort of a warmup; then we can talk about how our real lower bound, \Cref{thm:lb-ptf} below, improves on this in various ways: it works over a wider range of domains/product distributions, it gets the tight $n^{d/2}$ bound, it uses recent high tech Devroye et al machinery (we can mention how the $\Omega(n^{d/4})$ lower bound uses only simple linear algebra, essentially the idea from \href{https://www.cs.yale.edu/homes/aspnes/papers/stoc91voting.pdf}{the old ABFR paper)}.
%Or perhaps this discussion / pointer to the easy warmup can go into the intro of the whole paper rather than the beginning of this section - maybe that's a better place for it?}



\begin{theorem} \label{thm:lb-ptf}

Let $(\R^n, \mun)$ be a $(2,\red{\text{TODO}})$-hypercontractive distribution, and let $d \geq 1$ be a fixed constant. 
Let $A$ be any algorithm which is given access to samples from an unknown distribution ${\cal D}$ and has the following performance guarantee:
\begin{enumerate}
	\item If ${\cal D}=\mun$, then with probability at least $9/10$ the algorithm outputs ``un-truncated'';
	\item If ${\cal D}=\mun|_f$ where $f:\R^n\to\{0,1\}$ is an unknown degree-$d$ PTF with $\vol(f) \in [1/2 - o(1),1/2 + o(1)]$, then with probability at least $9/10$ the algorithm outputs ``truncated.''
\end{enumerate}
Then $A$ must use at least $\Omega(n^{d/2})$ samples from ${\cal D}$.

\end{theorem}


\red{TODO: high-level summary of LB. Introduce the ``un-truncated'' and ``truncated'' distributions $\calD_u$ and $\calD_t:=\calD_t(d)$ (cf. \Cref{fig:ptf-dist}).}



	

\subsection{Useful Preliminaries}
\label{subsec:lb-prelims}

We first recall a recent upper bound on the total variation distance between $n$-dimensional Gaussians due to Devroye, Mehrabian and Reddad \cite{DMR20}.

\begin{theorem} 
[Theorem~1.1 of \cite{DMR20}]  \label{thm:DMR20}
Let $\Sigma_1,\Sigma_2$ be two $m \times m$ positive definite covariance matrices and let $\lambda_1,\dots,\lambda_m$ be the eigenvalues of $\Sigma_1^{-1} \Sigma_2 - I_m$. Then
\[
\dtv\pbra{N(0^m,\Sigma_1),N(0^m,\Sigma_2)} \leq {\frac 3 2} \cdot \min\left\{1,\sqrt{\lambda_1^2 + \cdots + \lambda_m^2}\right\} 
\]
\end{theorem}

\begin{figure}

\centering

\fbox{\parbox{0.75\textwidth}{
\begin{enumerate}
	\item Draw the vector $\pbra{\wh{\bp}(\alpha)}_{\alpha \in {n\choose d}} =: \wh{\bp} \sim N(0, 1)^{{n\choose d}}$.
	\item Set \[\bp(x) := \sum_{{\substack{\alpha \in \zo^n\\|\alpha| = d}}} \wh{\bp}(\alpha)\chi_\alpha(x),\]
	and output the degree-$d$ PTF $\boldf(x) := \sign(\bp(x))$.  
\end{enumerate}
}}

\caption{A draw $\boldf$ from the distribution $\calD_t:=\calD_t(d)$}
\label{fig:ptf-dist}

\end{figure}


We will also require \Cref{lemma:balanced} which shows that a random PTF $\boldf$ drawn from $\calD_t := \calD_t(d)$ (see \Cref{fig:ptf-dist}) is close to being balanced with high probability.

\begin{lemma} \label{lemma:balanced}
For $\boldf\sim\calD_t$, we have with probability at least $1-o(1)$ that 
\[\vol(\boldf) \in \left[\frac{1}{2} - o(1), \frac{1}{2} + o(1)\right].\]
\end{lemma}

The proof of \Cref{lemma:balanced} will make use of the following well-known fact characterizing the probability that two vectors are both satisfying assignments of a random origin-centered LTF that has Gaussian coordinates. The fact follows immediately from spherical symmetry of the standard Gaussian distribution, and is sometimes known as ``Sheppard's formula'' (see Section 11.1 of \cite{ODonnell2014}).

\begin{fact} \label{fact:gaussian}
Let $u,v$ be unit vectors in $\R^n$.
We have
\[
\Prx_{\bg \sim N(0,I_n)}[\bg \cdot u \geq 0 \text{~and~}
\bg \cdot v \geq 0]
=
{\frac 1 2} - {\frac {\arccos(u \cdot v)}{2 \pi}}.
\]
\end{fact}

We now turn to the proof of \Cref{lemma:balanced}.\snote{\red{TODO:} Say that we assume WLOG that the distribution is CENTERED and that the linear Fourier coefficients are $x_i$. This I think is without loss of generality because hypercontractivity is scale-invariant?}

\begin{proofof}{\Cref{lemma:balanced}}
\snote{(Note to myself) Our basis functions right now don't make any assumptions about odd-ness versus even-ness, but I am pretty sure we don't need to worry about this.}\pink{If $d$ is odd then $p(-x)=-p(x)$ (i.e. $p$ is an odd function); since for any fixed $x$ we have that $p(x)=0$ with probability 0, it follows that $\vol(\boldf)=1/2$ with probability $1$ for odd $d$.  So in the rest of the argument we may suppose $d$ is even (though the argument we give will work for all $d \geq 1$, even or odd).}

Suppose $\boldf(x) := \mathbf{1}\cbra{\bp(x) \geq 0}$ is drawn from $\calD_t := \calD_t(d)$. We first observe that $\E[\vol(\boldf)]=1/2$. This is because
\begin{align*}
\E[\vol(\boldf)]&=
\Ex_{\bp}\left[
\Prx_{\bx \sim \mun}[\bp(\bx)\geq 0]\right]
=
\Ex_{\bx\sim\mun}\left[
\Prx_{\bp}\left[
\bp(\bx) \geq 0
\right]\right] = 1/2,
\end{align*}
where the last equality is because for each $x \in (\R^n \setminus 0^n)$ we have $\Prx[\bp(x) \geq 0]=1/2$ where the distribution over $\bp$ is as described in \Cref{fig:ptf-dist}. 

In order to show that $\vol(\boldf)$ is concentrated around $1/2$, we will upper bound the variance of $\vol(\boldf)$ and then appeal to Chebyshev's inequality. To start, we have 
\[
\Var[\vol(\boldf)] =
\Ex[\vol(\boldf)^2] - \Ex[\vol(\boldf)]^2
=
\Ex[\vol(\boldf)^2] - {\frac 1 4},
\]
so our goal is to show that $\Ex[\vol(\boldf)^2]$ is $1/4 + o(1)$.
\shivam{Here.}
\begin{align}
\Ex[\vol(\boldf)^2] &=
\Ex_{\bp}\left[
\Prx_{\bx \sim \mun}\left[\bp(\bx)\geq 0 \right]^2
\right]\nonumber \\
&=
\Ex_{\bp}\left[
\Prx_{\bx,\by \sim \mun}\left[\bp(\bx)\geq 0 \text{~and~}\bp(\by)\geq 0\right]
\right]\nonumber \\
&=
\Ex_{\bx,\by \sim \mun}\left[
\Prx_{\bp}\left[\bp(\bx) \geq 0 \text{~and~}\bp(\by)\geq0\right]
\right]\nonumber \\
&=
\Ex_{\bx,\by \sim \mun}\left[
\Prx_{\bp}\left[\sum_{S \in {[n] \choose d}} \widehat{\bp}(S) \bx_S \geq 0 \text{~and~}
\sum_{S \in {[n] \choose d}} \widehat{\bp}(S) \by_S \geq 0\right]
\right]\nonumber \\
&=
\Ex_{\bx,\by \sim \mun}\left[
\Prx_{\widehat{\bp} \sim N(0,1)^{[n] \choose d}}
\left[
\widehat{\bp} \cdot \Phi(\bx) \geq 0 \text{~and~}
\widehat{\bp} \cdot \Phi(\by) \geq 0
\right]
\right]. \label{eq:rutabaga}
\end{align}
\snote{Introduce the $\Phi$ notation; do we have a normalization issue?}
For any two vectors $x,y \in \bn$ we have that $\Phi(x),\Phi(y)$ are vectors in $\bits^{{n \choose d}}$.
Let us write $\Phi'(x)$ to denote ${\Phi(x)}/{\sqrt{{n \choose d}}}$, so $\Phi'(x)$ is $\Phi(x)$ normalized to be a unit vector in $\R^{{n \choose d}}.$ By \Cref{fact:gaussian} we have that
\begin{align}
(\ref{eq:rutabaga}) &=
\Ex_{\bx,\by \sim \bn}\left[
{\frac 1 2} - {\frac {\arccos(\Phi'(x) \cdot \Phi'(y))}{2 \pi}}
\right]. \label{eq:pumpkin}
\end{align}

Let
\[
h(x,y) := \Phi'(x) \cdot \Phi'(y) = {\frac {\sum_{S \in {[n] \choose d}} x_S y_S}{{n \choose d}}}.
\]
We see that $h(x,y)$ is a degree-$2d$ homogeneous polynomial with ${n \choose d}$ Fourier coefficients each of which is ${n \choose d}^{-1}$, so $\E_{\bx,\by \sim \bn}[h(\bx,\by)]=0$ and \red{$\Var[h]=\|h\|_2^2={n \choose d} \cdot {n \choose d}^{-2} = {n \choose d}^{-1}$}.
It follows from Chebyshev's inequality that
\[
\Pr\left[h(x,y) > t / {n \choose d}^{1/2}\right] \leq 1/t^2,
\]
so in particular we have that $\Pr_{\bx,\by \sim \bn}[\Phi'(\bx) \cdot \Phi'(\by) > {n \choose d}^{-1/3}] \leq {n \choose d}^{-1/3}.$
Since ${\frac 1 2} - {\frac {\arccos(\Phi'(x) \cdot \Phi'(y))}{2 \pi}}$ is always at most $1/2$, we get that 
\begin{align*}
(\ref{eq:pumpkin}) &\leq 
\left({\frac 1 2} - {\frac {\arccos({n \choose d}^{-1/3})}{2\pi}}\right) 
+
{\frac 1 2} \cdot \Prx_{\bx,\by \sim \bn}\left[\Phi'(\bx) \cdot \Phi'(\by) > {n \choose d}^{-1/3}\right]\nonumber\\
&\leq \left({\frac 1 2} - {\frac {\arccos({n \choose d}^{-1/3})}{2\pi}}\right) 
+ {\frac 1 2}\cdot {n \choose d}^{-1/3}\nonumber\\
&\leq {\frac 1 2} - {\frac {\pi/2 - 2 {n \choose d}^{-1/3}}{2 \pi}} + {\frac 1 2}\cdot {n \choose d}^{-1/3}\nonumber\\
&\leq {\frac 1 4} + C {n \choose d}^{-1/3}
\end{align*}
for an absolute constant $C>0$.
So $\Var[\vol(\boldf)] \leq C{n \choose d}^{-1/3}$, and hence Chebyshev's inequality tells us that $|\vol(\boldf) - {\frac 1 2}| \geq {n \choose d}^{-1/12}$ with probability at most $O({n \choose d}^{-1/6})=o(1),$ as claimed.
\end{proofof}


\subsection{Proof of \Cref{thm:lb-ptf}}
\label{subsec:lb-proof}

==> sn-backup/baseline-distinguisher.tex <==
\section{BASELINE}
\label{appendix:baseline-distinguisher}

==> sn-backup/dkp-sosa-thing.tex <==
\section{Distinguishing LTF Truncation of Log-Concave Distributions}
\label{appendix:dkp-sosa}

In the specific setting when the background distribution is the standard $n$-dimensional Gaussian distribution, De, Nadimpalli, and Servedio~\red{TODO:SODA citation} obtained a $O_\eps(\sqrt{n})$ distinguisher but with a worse $\epsilon$-dependence. \red{TODO: write this up more clearly.}

==> sn-backup/intro.tex <==
\section{Introduction}
\label{sec:intro}

==> sn-backup/lb.tex <==
\section{An $\Omega(n^{d/2})$-Sample Lower Bound for Distinguishing PTFs}
\label{sec:lb}

\red{TODO: Prose saying this is what we will prove here.}

\

{\large \shivam{I think taking multilinear polynomials works for us?}}


\begin{theorem} \label{thm:lb-ptf}

Let $(\R^n, \mun)$ be a \red{$TODO$}-hypercontractive distribution, and let $d \geq 1$ be a fixed constant. 
Let $A$ be any algorithm which is given access to samples from an unknown distribution ${\cal D}$ and has the following performance guarantee:

\begin{enumerate}

\item If ${\cal D}=\mun$, then with probability at least $9/10$ the algorithm outputs ``un-truncated'';

\item If ${\cal D}=\mun|_f$ where $f:\R^n\to\{0,1\}$ is an unknown degree-$d$ PTF $f(x)=\sign(p(x))$ with $\vol(f) \in [1/2 - o(1),1/2 + o(1)]$, then with probability at least $9/10$ the algorithm outputs ``truncated.''

\end{enumerate}

Then $A$ must use at least $\Omega(n^{d/2})$ samples from ${\cal D}$.

\end{theorem}


\red{TODO: high-level summary of LB}


\begin{figure}

\centering

\fbox{\parbox{0.75\textwidth}{
\begin{enumerate}
	\item Draw the vector $\pbra{\wh{\bp}(\alpha)}_{\alpha \in {n\choose d}} =: \wh{\bp} \sim N(0, 1)^{{n\choose d}}$.
	\item Set \[\bp(x) := \sum_{\alpha \in {n\choose d}} \wh{\bp}(\alpha)\chi_\alpha(x),\]
	and output the degree-$d$ PTF $\boldf(x) := \sign(\bp(x))$.  
\end{enumerate}
}}

\caption{The Distribution $\PTFd$}
\label{fig:ptf-no-dist}

\end{figure}
	

\subsection{Useful Preliminaries}
\label{subsec:lb-prelims}

We first recall a recent upper bound on the total variation distance between $n$-dimensional Gaussians due to Devroye, Mehrabian and Reddad \cite{DMR20}.

\begin{theorem} 
[Theorem~1.1 of \cite{DMR20}]  \label{thm:DMR20}
Let $\Sigma_1,\Sigma_2$ be two $m \times m$ positive definite covariance matrices and let $\lambda_1,\dots,\lambda_m$ be the eigenvalues of $\Sigma_1^{-1} \Sigma_2 - I_m$. Then
\[
\dtv(N(0^m,\Sigma_1),N(0^m,\Sigma_2)) \leq {\frac 3 2} \cdot \min\left\{1,\sqrt{\lambda_1^2 + \cdots + \lambda_m^2}\right\} 
\]
\end{theorem}


We will also require the following lemma which shows that a random PTF $\boldf\sim\PTFd$ (see \Cref{fig:ptf-dist}) is with high probability close to being balanced. 

\begin{lemma} \label{lemma:balanced}
Let $\boldf \sim {\cal PTF}_d$. With probability at least $1-o(1)$ we have 
\[\vol(\boldf) \in \left[\frac{1}{2} - o(1), \frac{1}{2} + o(1)\right].\]
\end{lemma}

\red{
\begin{proof}
If $d$ is odd then $p(-x)=-p(x)$ (i.e. $p$ is an odd function); since for any fixed $x$ we have that $p(x)=0$ with probability 0, it follows that $\vol(\boldf)=1/2$ with probability $1$ for odd $d$.  So in the rest of the argument we may suppose $d$ is even (though the argument we give will work for all $d \geq 1$, even or odd).

We first observe that $\E[\vol(\boldf)]=1/2$: this is because
\begin{align*}
\E[\vol(\boldf)]&=
\Ex_{\bp}\left[
\Prx_{\bx \sim \bn}[\bp(\bx)\geq 0]\right]
=
\Ex_{\bx}\left[
\Prx_{\bp}\left[
\bp(\bx) \geq 0
\right]\right] = 1/2,
\end{align*}
where the last equality is because for each $x \in (\R^n \setminus 0^n)$ we have $\Prx_{\bp}[\bp(x) \geq 0]=1/2.$

Next, we upper bound the variance of $\vol(\boldf)$. We have
\[
\Var[\vol(\boldf)] =
\Ex[\vol(\boldf)^2] - \Ex[\vol(\boldf)]^2
=
\Ex[\vol(\boldf)^2] - {\frac 1 4},
\]
so our goal is to show that $\Ex[\vol(\boldf)^2]$ is $1/4 + o(1)$.
\begin{align}
\Ex[\vol(\boldf)^2] &=
\Ex_{\bp}\left[
\Prx_{\bx \sim \bn}[\bp(\bx)\geq 0]^2
\right]\nonumber \\
&=
\Ex_{\bp}\left[
\Prx_{\bx,\by \sim \bn}[\bp(\bx)\geq 0 \text{~and~}\bp(\by)\geq 0]
\right]\nonumber \\
&=
\Ex_{\bx,\by \sim \bn}\left[
\Prx_{\bp}[\bp(\bx) \geq 0 \text{~and~}\bp(\by)\geq0]
\right]\nonumber \\
&=
\Ex_{\bx,\by \sim \bn}\left[
\Prx_{\bp}\left[\sum_{S \in {[n] \choose d}} \widehat{\bp}(S) \bx_S \geq 0 \text{~and~}
\sum_{S \in {[n] \choose d}} \widehat{\bp}(S) \by_S \geq 0\right]
\right]\nonumber \\
&=
\Ex_{\bx,\by \sim \bn}\left[
\Prx_{\widehat{\bp} \sim N(0,1)^{[n] \choose d}}
\left[
\widehat{\bp} \cdot \Phi(\bx) \geq 0 \text{~and~}
\widehat{\bp} \cdot \Phi(\by) \geq 0
\right]
\right]. \label{eq:rutabaga}
\end{align}

We recall the following fact characterizing the probability that two vectors are both satisfying assignments of a random origin-centered LTF that has Gaussian coordinates. (The fact follows immediately from spherical symmetry of the standard Gaussian distribution.)

\begin{fact} \label{fact:gaussian}
Let $u,v$ be unit vectors in $\R^N$.
We have
\[
\Prx_{\bg \sim N(0,1)^N}[\bg \cdot u \geq 0 \text{~and~}
\bg \cdot v \geq 0]
=
{\frac 1 2} - {\frac {\arccos(u \cdot v)}{2 \pi}}
\]
\end{fact}

For any two vectors $x,y \in \bn$ we have that $\Phi(x),\Phi(y)$ are vectors in $\bits^{{n \choose d}}$.
Let us write $\Phi'(x)$ to denote ${\Phi(x)}/{\sqrt{{n \choose d}}}$, so $\Phi'(x)$ is $\Phi(x)$ normalized to be a unit vector in $\R^{{n \choose d}}.$ By \Cref{fact:gaussian} we have that
\begin{align}
(\ref{eq:rutabaga}) &=
\Ex_{\bx,\by \sim \bn}\left[
{\frac 1 2} - {\frac {\arccos(\Phi'(x) \cdot \Phi'(y))}{2 \pi}}
\right]. \label{eq:pumpkin}
\end{align}

Let
\[
h(x,y) := \Phi'(x) \cdot \Phi'(y) = {\frac {\sum_{S \in {[n] \choose d}} x_S y_S}{{n \choose d}}}.
\]
We see that $h(x,y)$ is a degree-$2d$ homogeneous polynomial with ${n \choose d}$ Fourier coefficients each of which is ${n \choose d}^{-1}$, so $\E_{\bx,\by \sim \bn}[h(\bx,\by)]=0$ and \red{$\Var[h]=\|h\|_2^2={n \choose d} \cdot {n \choose d}^{-2} = {n \choose d}^{-1}$}.
It follows from Chebyshev's inequality that
\[
\Pr\left[h(x,y) > t / {n \choose d}^{1/2}\right] \leq 1/t^2,
\]
so in particular we have that $\Pr_{\bx,\by \sim \bn}[\Phi'(\bx) \cdot \Phi'(\by) > {n \choose d}^{-1/3}] \leq {n \choose d}^{-1/3}.$
Since ${\frac 1 2} - {\frac {\arccos(\Phi'(x) \cdot \Phi'(y))}{2 \pi}}$ is always at most $1/2$, we get that 
\begin{align*}
(\ref{eq:pumpkin}) &\leq 
\left({\frac 1 2} - {\frac {\arccos({n \choose d}^{-1/3})}{2\pi}}\right) 
+
{\frac 1 2} \cdot \Prx_{\bx,\by \sim \bn}\left[\Phi'(\bx) \cdot \Phi'(\by) > {n \choose d}^{-1/3}\right]\nonumber\\
&\leq \left({\frac 1 2} - {\frac {\arccos({n \choose d}^{-1/3})}{2\pi}}\right) 
+ {\frac 1 2}\cdot {n \choose d}^{-1/3}\nonumber\\
&\leq {\frac 1 2} - {\frac {\pi/2 - 2 {n \choose d}^{-1/3}}{2 \pi}} + {\frac 1 2}\cdot {n \choose d}^{-1/3}\nonumber\\
&\leq {\frac 1 4} + C {n \choose d}^{-1/3}
\end{align*}
for an absolute constant $C>0$.
So $\Var[\vol(\boldf)] \leq C{n \choose d}^{-1/3}$, and hence Chebyshev's inequality tells us that $|\vol(\boldf) - {\frac 1 2}| \geq {n \choose d}^{-1/12}$ with probability at most $O({n \choose d}^{-1/6})=o(1),$ as claimed.
\end{proof}
}

\subsection{Proof of \Cref{thm:lb-ptf}}
\label{subsec:lb-proof}

==> sn-backup/prelims.tex <==
\section{Preliminaries}
\label{sec:prelims}


We write $\N := \{0,1,\ldots\}$. Let $(\R^n, \calD)$ be a probability space. For $n\in\N$, we write $L^2(\R^n, \calD)$ for the (real) inner-product space of functions $f:\R^n\to\R$ with the inner product 
\[\abra{f,g} := \Ex_{\bx\sim\calD}\sbra{f(\bx)\cdot g(\bx)}.\]
Here $\mun$ denotes the product probability distribution on $\R^n$. 
%\red{We assume throughout that $L^2(\R, \mu)$ is a separable space (and consequently so is $L^2(\R^n, \mun)$)}.\footnote{Recall that a topological space is said to be \emph{separable} if it contains a countable dense subset.} 
We write 
\[\|f\|_q := \Ex_{\bx\sim\calD}\sbra{|f(\bx)|^q}^{1/q}.\]
In particular, for $f:\R^n\to\{0,1\}$, we write $\vol(f) := \|f\|_1 = \Ex[f(\bx)]$ where $\bx\sim\calD$. 

We say that a function $f:\R^n\to\zo$ is a \emph{degree-$d$ polynomial threshold function (PTF)} if there exists a degree-$d$ polynomial $p:\R^n\to\R$ such that 
\[f(x) = \Indicator\{p(x) \geq 0\}.\]
The primary class of distributions we will consider throughout is that of truncations of an i.i.d. product distribution $\mun$ by a degree-$d$ PTF of volume at least inverse exponential in $n$; more precisely, we will consider the following class of truncations:
\begin{equation} \label{eq:class-def}
	\Pptf := \cbra{\mun\mid_{f^{-1}(1)} \ : f \text{ is a degree-$d$ PTF with } \vol(f) \geq 2^{-\sqrt{n}} }.
\end{equation}
We note that we can replace $2^{-\sqrt{n}}$ in the definition of $\Pptf$ above by $c^{-\sqrt{n}}$ for any arbitrary constant $c$; we choose to work with the above definition for convenience. We also assume throughout that the $d$---the degree of the PTFs under consideration---is a fixed constant independent of the ambient dimension $n$. 

\subsection{Harmonic Analysis over Product Spaces}
\label{subsec:fourier-101}

Our notation and terminology in this section closely follow those of O'Donnell~\cite{ODonnell2014}; in particular, we refer the reader to Chapter~8 of~\cite{ODonnell2014} for further background. 

\begin{definition}
	A \emph{Fourier basis} for $L^2(\R, \mu)$ is an orthonormal basis $\calB = \{\chi_0,\chi_1, \ldots\}$ with $\chi_0 \equiv 1$. 
\end{definition}

It is well known that $L^2(\R, \mu)$ is separable and hence has a Fourier basis. We can obtain a Fourier basis for $L^2(\R^n, \mun)$ by taking all possible $n$-fold products of elements of $\calB$; more formally, for a multi-index $\alpha\in\N^n$, we define 
\[\chi_{\alpha}:=\prod_{i=1}^n \chi_{\alpha_i}.\]
Then the collection 
$\calB_n := \cbra{ \chi_\alpha : \alpha_i \in \N^n}$
forms a Fourier basis for $L^2(\R^n, \mun)$; this lets us write $f\in L^2(\R^n, \mun)$ as $f = \sum_{\alpha\in\N^n} \wh{f}(\alpha)\chi_{\alpha}$ where  
\[\wh{f}(\alpha) := \abra{f, \chi_\alpha}\] 
is the \emph{Fourier coefficient of $f$ on $\alpha$}.

We can assume without loss of generality that the basis elements $\chi_\alpha$ are polynomials; this is because a polynomial basis can be obtained for $L^2(\R, \mu)$ by running the Gram-Schmidt process and then extending it to a basis for $L^2(\R^n,\mun)$ by taking products.

\begin{remark}
While the Fourier coefficients $\{\wh{f}(\alpha)\}$ depend on the choice of basis $\cbra{\chi_\alpha}$, we will always work with some fixed (albeit arbitrary) polynomial basis, and hence there should be no ambiguity in referring to the coefficients as though they were unique.
\end{remark}

As a consequence of orthonormality, we get that for any $f\in L^2(\R^n,\mun)$, we have 
\[\Ex_{\bx\sim\mun}\sbra{f(\bx)} = \wh{f}(0^n) \qquad\text{and}\qquad \|f\|_2^2 = \sum_{\alpha\in\N^n} \wh{f}(\alpha)^2,\]
with the latter called \emph{Parseval's formula}.
We also have \emph{Plancharel's formula}, which says that 
\[\abra{f, g} = \sum_{\alpha\in\N^n} \wh{f}(\alpha)\wh{g}(\alpha).\]

\begin{notation}
Given a multi-index $\alpha\in\N^n$, we write 
\[\#\alpha := \abs{\cbra{i : \alpha_i \neq 0 }} \qquad\text{and}\qquad |\alpha| := \sumi \alpha_i.\]
Note that given a polynomial basis $\{\chi_\alpha\}$, we can assume that $\deg(\chi_{\alpha}) = |\alpha|$. We also write 
\[\bW^{=k}[f] := \sum_{|\alpha| = k}\wh{f}(\alpha)^2,\]
with $\bW^{\leq k}[f]$ defined similarly.
\end{notation}


\subsection{Hypercontractive Distributions}
\label{subsec:hypercontractive}

The primary analytic tools we will require in both our upper and lower bounds are consequences of \emph{hypercontractive} estimates for functions in $L^2(\R^n,\mun)$; we refer the reader to Chapters~9 and 10 of~\cite{ODonnell2014} for further background on hypercontractivity and its applications. 

\begin{definition} \label{def:hypercontractive-domain}
	For $2\leq q\leq \infty$, we say that $(\R^n, \calD)$ is \emph{$(2, q)$-hypercontractive} if for every (multivariate) degree-$d$ polynomial $p : \R\to\R$ we have 
	\begin{equation} \label{eq:general-bonami}
		\|p\|_q \leq C_q(\mu)^d\cdot \|p\|_2
	\end{equation}
	with $C_q(\mu)$ satisfying
	\begin{equation} \label{eq:hyp-constant-growth}
		C_q(\mu) \leq K\sqrt{q}
%		\snote{We need this constraint because otherwise I don't think we get the $\ln(1/\alpha)$ saving in the level-$k$ inequality.}
	\end{equation}
	for some absolute constant $K$.
\end{definition}

\ignore{
It is easy to check that the hypercontractivity tensorizes; more formally, we have the following via a straightforward inductive argument:

\begin{proposition} \label{prop:tensorization}
	If $(\R, \mu)$ is $(2,q)$-hypercontractive for some $2\leq q\leq \infty$, then so is $(\R^n, \mun)$ for all $n\in\N$, i.e. for every multivariate degree-$d$ polynomial $p:\R^n\to\R$, we have
	\[\|p\|_q \leq C_q(\mu)^d\cdot \|p\|_2\]
	for some absolute constant $C_q(\mu)$ satisfying \Cref{eq:hyp-constant-growth}.
\end{proposition}

\begin{proof}
  We shall prove the proposition by an induction on $n$.
  For the base case when $n=1$, the proposition immediately follows
  from the $(2,q)$-hypercontractivity of $(\mathbb{R},\mu)$.
  We then do the induction step.
  Suppose for some integer $k\geq 1$,
  the proposition holds for all $n\in[1,k]$. We shall
  prove that the proposition also holds when $n=k+1$.
  Since $p$ is a degree-$d$ polynomial on variables $x_1,\ldots,x_n$,
  we can write $p(\bx)$ as $p(\bx) = x_n f(\bx) + g(\bx)$ such that
  $f(\bx)$ has degree $\leq d-1$, $g(\bx)$ has degree $\leq d$, and neither
  $f(\bx)$ or $g(\bx)$ depends on $x_n$.
  Now we write
  \begin{align*}
    \Ex_{\bx\sim\mun}\sbra{p(\bx)^2} = &
    \Ex_{\bx\sim\mun}\sbra{ (x_n f(\bx) + g(\bx))^2 } \\
    = &
    \Ex_{\bx\sim\mun}\sbra{ x_n^2 f^2(\bx) } +
    \Ex_{\bx\sim\mun}\sbra{ 2 x_n f(\bx) g(\bx) } +
    \Ex_{\bx\sim\mun}\sbra{ g^2(\bx) } \\
    & \qquad \text{(Expanding and linearity of expectation)}
    \\
    = & \Ex_{\bx\sim\mun}\sbra{ x_n^2 f^2(\bx) } +
    \Ex_{\bx\sim\mun}\sbra{ g^2(\bx) } \\
    & \qquad \text{($x_n$ is independent of $f(\bx)$ and $g(\bx)$ and $\Ex\sbra{x_n} = 0$)} \\
    = & \Ex_{\bx\sim\mun}\sbra{ x_n^2}
    \Ex_{\bx\sim\mun}\sbra{ f^2(\bx) } +
    \Ex_{\bx\sim\mun}\sbra{ g^2(\bx) } \\
    & \qquad \text{($x_n$ is independent of $f(\bx)$).} \\
  \end{align*}
  On the other hand, we have
  \begin{align*}
    \Ex_{\bx\sim\mun}\sbra{|p(\bx)|^q}^{1/q} = &
    \Ex_{\bx\sim\mun}\sbra{ (x_n f(\bx) + g(\bx))^q }^{1/q} \\
    \leq &
    \Ex_{\bx\sim\mun}\sbra{ |x_n f(\bx)|^q }^{1/q} +
    \Ex_{\bx\sim\mun}\sbra{ |g(\bx)|^q }^{1/q}
    \qquad \text{(Triangle inequality)}
    \\
    = & \Ex_{\bx\sim\mun}\sbra{ |x_n|^q }^{1/q}
    \Ex_{\bx\sim\mun}\sbra{ |f(\bx)|^q }^{1/q} +
    \Ex_{\bx\sim\mun}\sbra{ |g(\bx)|^q }^{1/q} \\
    & \qquad \text{($x_n$ is independent of $f(\bx)$)} \\
    \leq & C_q(\mu) \Ex_{\bx\sim\mun}\sbra{ x_n^2 }^{1/2}\cdot
    C_q(\mu)^{d-1} \Ex_{\bx\sim\mun}\sbra{ f^2(\bx) }^{1/2} +
    C_q(\mu)^{d} \Ex_{\bx\sim\mun}\sbra{ g^2(\bx) }^{1/2} \\
    & \qquad \text{(by $(2,q)$-hypercontractivity of $x_n$ and induction hypothesis)} \\
    \leq & C_q(\mu)^d \left( \Ex_{\bx\sim\mun}\sbra{ x_n^2}
    \Ex_{\bx\sim\mun}\sbra{ f^2(\bx) } +
  \Ex_{\bx\sim\mun}\sbra{ g^2(\bx) } \right)^{1/2}
  \end{align*}
  {\color{red} TODO: Last line does not follow}
\end{proof}
}

We note that \Cref{def:hypercontractive-domain} is not the standard definition of a hypercontractive product distribution (cf. Chapter~10 of \cite{ODonnell2014}), but is in fact a consequence of hypercontractivity that is sometimes referred to as the ``Bonami lemma.'' The guarantees of \Cref{eq:general-bonami,eq:hyp-constant-growth} are all we require for our purposes, and so we instead work with the slightly this slightly more restrictive definition; see \Cref{table:hypercontractive} for examples of hypercontractive distributions with accompanying hypercontractivity constants $C_q(\mu)$.\snote{TODO: Check if things are ok for spherical harmonics (a non-product distribution)!}

We next turn to record several useful consequences of hypercontractivity which will be crucial to the analysis of our estimator in \Cref{sec:ub} as well as that of our lower bound in \Cref{sec:lb}. The following proposition informally says that low-degree polynomials are reasonably anti-concentrated under hypercontractive distributions. 

{\renewcommand{\arraystretch}{1.5}
\begin{table}[]
\begin{center}
\begin{tabular}{@{}lll@{}}
\toprule
                                         & $C_q(\mu)$ &   Reference       \\ \midrule
Standard Gaussian Distribution $N(0,I_n)$                    &      $\sqrt{q-1}$      &      Proposition~5.48 of~\cite{Aubrun2017}     \\ 
Uniform Measure on $\bn$                       &    $\sqrt{q-1}$        &       Theorem~9.21 of~\cite{ODonnell2014}    \\
Finite Product Domains $(\Omega^n, \mun)$ &  $\sqrt{\frac{q}{2\min (\mu)}}$          &      \cite{Wolff2007} and Fact~2.8 of~\cite{aushas09}     \\
\bottomrule
\end{tabular}
\caption{Examples of distributions that are $(2,q)$-hypercontractive for all $2\leq q\leq \infty$, along with their accompanying hypercontractivity constants. Here $\min(\mu)$ denotes the minimal non-zero probability of any element in the support of the (finitely supported) distribution $\mu$.}
\label{table:hypercontractive}
\end{center}
\end{table} 
}


\begin{proposition}[Anti-concentration of low-degree polynomials]
  Suppose $(\R^n, \calD)$ is $(2,q)$-hypercontractive. Then for any degree-$d$ polynomial $p(\bx)$, we have
  \begin{align*}
    \Prx\sbra{|p(\bx)| > t \norm{p}_2} \geq
    \left( (1 - t^2) / C_q(\mu)^{2d} \right)^{\frac{q}{q-2}}.
  \end{align*} 
\end{proposition}

\begin{proof}
  First, note that 
  \begin{align*}
    \Prx\sbra{|p(\bx)| > t \norm{p}_2} =
    & \Prx\sbra{p(\bx)^2 - t^2 \norm{p}_2^2 > 0}.
  \end{align*}
  This lets us write
  \begin{align*}
    \Ex\sbra{p(x)^2} &= \Ex\sbra{p(x)^2\cdot 1_{p(x)^2\leq t^2 \norm{p}_2^2}}
    +
    \Ex\sbra{p(x)^2\cdot 1_{p(x)^2 > t^2 \norm{p}_2^2}} \\ 
    &\leq t^2 \norm{p}_2^2 + 
    \Ex\sbra{(p(x)^2)^{q/2}}^{2/q}
    \Prx\sbra{p(x)^2 > t^2 \norm{p}_2^2}^{1-2/q} \\ 
    &= t^2 \norm{p}_2^2 + 
    \|p\|_q^2\cdot
    \Prx\sbra{p(x)^2 > t^2 \norm{p}_2^2}^{1-2/q}
  \end{align*}
  where the inequality is due to  H\"older's.
  By rearranging, we get
  \begin{align*}
    \Prx\sbra{p(x)^2 > t^2 \norm{p}_2^2} \geq
    & \left( (1 - t^2) \norm{p}_2^2 / \norm{p}_q^2 \right)^{\frac{q}{q-2}} \\ \geq
    & \left( (1 - t^2) / C_q(\mu)^{2d} \right)^{\frac{q}{q-2}}
  \end{align*}
  as desired, where the second inequality follows from hypercontractivity.
\end{proof}

%\begin{proposition}[Anti-concentration of low-degree polynomials]
%  For any degree-$d$ polynomial $p(\bx)$, we have for any $\theta\in\mathbb{R}$
%  \begin{align*}
%    \Prx\sbra{|p(\bx) - \theta| > t \norm{p}_2} \geq
%    \left( (1 - t^2) / C_q(\mu)^{2d} \right)^{2}.
%  \end{align*}
%\end{proposition}

The following proposition bounds Fourier weight up to level $k$ (i.e. $\bW^{\leq k}[f]$) in terms of the bias (i.e. the degree-$0$ Fourier coefficient) of the function. We note that this lemma is sometimes known as ``Chang's Lemma'' or ``Talagrand's Lemma'' \cite{changs-lemma,Talagrand:96}; see also Section 9.5 of \cite{ODonnell2014}.

\begin{proposition}[Level-$k$ inequalities] \label{prop:level-k-inequalities}
	Let $(\R^n, \mun)$ be a probability space and $f : \R^n \to \zo$. If $(\R^n, \mun)$ is $(2, q)$-hypercontractive with $q := 2\log\pbra{\frac{1}{\vol(f)}}$, then for all $k\leq q$ we have
	\[\bW^{\leq k}[f] \leq K^{k}\cdot \vol(f)^2\cdot \pbra{\log\pbra{\frac{1}{\vol(f)}}}^k\]
	where $K$ is an absolute constant. 
\end{proposition}

\begin{proof}
	Let $f^{\leq k} := \sum_{|\alpha| \leq k} \wh{f}(\alpha)\chi_\alpha$ and note that $\bW^{\leq k}[f] = \langle f, f^{\leq k} \rangle$. By H\"older's inequality, we have
	\begin{equation} \label{eq:level-k-holder}
		\langle f, f^{\leq k} \rangle \leq \|f\cdot f^{\leq k}\|_1 \leq \|f\|_{s}\cdot\|f^{=k}\|_{t}
	\end{equation}
	for all $1\leq s, t \leq \infty$ with $1/s + 1/t = 1$. We will take 
	\[t :=  \frac{q}{k} = \frac{2}{k}\log\pbra{\frac{1}{\vol(f)}},\]
	noting that $t\geq 1$ as $k\leq q$. We next bound each term on the right hand side of \Cref{eq:level-k-holder} separately. First, note that 
	\begin{equation} \label{eq:holder-rhs-first-term}
		\|f\|_{s} \leq \vol(f)^{1/s} = \vol(f)^{1- 1/t} 
	\end{equation}
	as $f(x) \in \zo$ and $s \geq 1$. 
	Furthermore, as $t\leq q$, we have by $(2,q)$-hypercontractivity that  
	\begin{equation} \label{eq:holdr-rhs-second-term}
		\|f^{\leq k}\|_{t} \leq \|f^{\leq k}\|_q \leq C_q(\mu)^k\cdot \|f^{\leq k}\|_2 = C_q(\mu)^k\cdot\sqrt{\bW^{\leq k}[f]}
	\end{equation}
	where the first inequality is due to monotonicity of norms. 
	Combining \Cref{eq:level-k-holder,eq:holder-rhs-first-term,eq:holdr-rhs-second-term} and rearranging, we get that 
	\begin{align*}
		\bW^{\leq k}[f] &\leq C_q(\mu)^{2k}\cdot \vol(f)^2 \cdot \pbra{\frac{1}{\vol(f)}}^{2/t}\\
		&\leq K_1^{2k} q^k\cdot \vol(f)^2 \cdot  \pbra{\frac{1}{\vol(f)}}^{k/\log(1/\vol(f))}\\
		&= K_2^{k}\cdot \vol(f)^2 \cdot \pbra{\log\pbra{\frac{1}{\vol(f)}}}^k
	\end{align*}
	where $K_1$ and $K_2$ are absolute constants, completing the proof. 
\end{proof}

\begin{remark}
	We note that the \Cref{prop:level-k-inequalities} also holds for bounded functions $f:\R^n\to[-1,1]$ rather than Boolean-valued functions with an identical proof, although we will not require this. 
\end{remark}

\snote{TODO: Write up the degree-$d$ Chernoff bound (used in lower bound)}





==> sn-backup/ub.tex <==
\section{An $O(n^{d/2})$-Sample Algorithm for Degree-$d$ PTFs}
\label{sec:ub}

In this section, we present a $O(n^{d/2})$-sample algorithm for distinguishing a hypercontractive product distribution $\mun$ from the $\mun$ truncated by the satisfying assignments of a degree-$d$ PTF. More precisely, we prove the following: 

\begin{theorem} \label{thm:ptf-ub}
Let $\mu$ be $(2, \red{\text{TODO}})$-hypercontractive. There is an algorithm, \PTF\newline (\Cref{alg:ptf}), with the following performance guarantee: Given any $\eps > 0$ and access to independent samples from any unknown distribution ${\cal D} \in \Pptf$, the algorithm uses \red{TODO} samples, runs in \red{TODO} time, and 
\begin{enumerate}

\item If ${\cal D}=\mun$, then with probability at least $9/10$ the algorithm outputs ``un-truncated;''

\item If $\dtv\pbra{\mun, \calD} \geq \eps$, then with probability at least $9/10$ the algorithm outputs ``truncated.''

\end{enumerate}
\end{theorem}

We note that a similar estimator\snote{It's not ``similar'' but ``identical''\ldots} has recently been used by Diakonikolas, Kane, and Pensia~\cite{DKP-SOSA} for the problem of \emph{Gaussian mean testing}. We also note that the~\cite{DKP-SOSA} analysis can be easily extended to give a $O_\eps(\sqrt{n})$-distinguishing algorithm for degree-$1$ truncation when the background distribution is an arbitrary log-concave distribution \emph{without any assumption on the volume of the truncating function} (cf. \Cref{eq:class-def}); we include a proof of this in \Cref{appendix:dkp-sosa}. 

\begin{algorithm}[t]
\caption{Distinguisher for General Convex Sets}
\label{alg:ptf}
\vspace{0.5em}
\textbf{Input:} $\calD\in\{\mun\}\cup\Pptf$\\[0.5em]
\textbf{Output:} ``Un-truncated'' or  ``truncated''

\ 

\PTF$(\calD)$:
\begin{enumerate}
    \item For $T =C\cdot n^{d/2}$, sample points $\x{1}, \ldots, \x{T} \sim \calD$. 
    \item Compute the statistic $\bM$ where 
    \[\bM := \frac{1}{T^2} \abra{\tx{i},\tx{j}} \qquad\text{with}\qquad \tx{i} := \pbra{\chi_{\alpha}(\x{i})}_{|\alpha|\leq d}.\]
    \item Output ``truncated'' if $\bM \geq \red{\text{TODO}}$
    	and ``un-truncated'' otherwise.
\end{enumerate}

\end{algorithm}



\begin{proofof}{\Cref{thm:ptf-ub}}
Throughout, we will write 
\[m := \#\cbra{\alpha\in\N^n : 1 \leq |\alpha| \leq d}.\]
We compute the mean and variance of the estimator $\bM$ in each case (i.e. when $\calD = \mun$ and when $\calD \in \Pptf$). 

\paragraph{Case 1: $\calD = \mun$.} When $\x{1},\ldots,\x{T}\sim\mun$, we have 
\begin{align}
	\Ex\sbra{\bM} &= \sum_{|\alpha|\leq d} \Ex\sbra{\chi_\alpha(\x{i})\cdot\chi_\alpha(\x{j})} \nonumber \\
	&= \sum_{|\alpha|\leq d} \Ex\sbra{\chi_\alpha(\x{i})}\Ex\sbra{\chi_\alpha(\x{j})} \nonumber \\
	&= 0, \label{eq:untrunc-means}
\end{align}
as $\x{i},\x{j}$ are independent samples and by the orthonormality of $\{\chi_{\alpha}\}$. Turning to the variance, we have 
\begin{align}
	\Var[\bM] &= {T\choose 2}^{-2}\pbra{\sum_{\substack{i<j\\k<l}} \Ex\sbra{\abra{\tx{i},\tx{j}}\abra{\tx{k},\tx{l}}} - \Ex\sbra{\abra{\tx{i},\tx{j}}}\Ex\sbra{\abra{\tx{k},\tx{l}}}} \label{eq:generic-variance}\\
	&= {T\choose 2}^{-2}\pbra{\sum_{\substack{i<j\\k<l}} \Ex\sbra{\abra{\tx{i},\tx{j}}\abra{\tx{k},\tx{l}}}}, \nonumber
\end{align}
as the second term in the summation is $0$ for every $i<j$ and $k<l$. (cf. \Cref{eq:untrunc-means}). We have the following cases:
\begin{enumerate}
	\item When $|\cbra{i,j} \cap \cbra{k,l}| = 0$, then 
	\[\Ex\sbra{\abra{\tx{i},\tx{j}}\abra{\tx{k},\tx{l}}} = \Ex\sbra{\abra{\tx{i},\tx{j}}}\Ex\sbra{\abra{\tx{k},\tx{l}}} = 0.\]

	\item When $|\cbra{i,j} \cap \cbra{k,l}| = 1$, because say $j = l$, then 
	\begin{align*}
		\Ex\sbra{\abra{\tx{i},\tx{j}}\abra{\tx{k},\tx{j}}} &= \Ex\bigg[\pbra{\tx{i}}^T {\tx{j}\pbra{\tx{j}}^T}\tx{k}\bigg]\\
		&= \Ex\bigg[\pbra{\tx{i}}^T\bigg]\Ex\bigg[{\tx{j}\pbra{\tx{j}}^T}\bigg]
\Ex\bigg[\tx{k}\bigg].
	\end{align*}
	However, once again by orthonormality, we have 
	\[
	\Ex\sbra{{\tx{j}\pbra{\tx{j}}^T}} = \mathrm{Id}_m
	\]
	where $\mathrm{Id}_m$ denotes the $m\times m$ identity matrix, and so 
	\[\Ex\sbra{\abra{\tx{i},\tx{j}}\abra{\tx{k},\tx{j}}} = \Ex\sbra{\abra{\tx{i},\tx{k}}} = 0.\]
	
	\item When $|\cbra{i,j} \cap \cbra{k,l}| = 2$, then proceeding as in the previous case, we have 
	\[\Ex\sbra{\abra{\tx{i},\tx{j}}\abra{\tx{i},\tx{j}}} = \Ex\sbra{\abra{\tx{i},\tx{i}}} = {m}.\]
\end{enumerate}
Putting everything together, we get that 
\begin{equation} \label{eq:var-untrunc}
	\Var[\bM] = {T\choose 2}^{-2} \pbra{ \sum_{\cbra{i,j} = \cbra{k,l}} \Ex\sbra{\abra{\tx{i},\tx{j}}\abra{\tx{i},\tx{j}}} } = O\pbra{\frac{m}{T^2}}.
\end{equation}

\paragraph{Case 2: $\dtv\pbra{\mun, \calD}\geq\eps$.} Suppose $\x{1},\ldots,\x{T}$ are drawn from $\mun\upharpoonright_{f^{-1}(1)}$ where $f:\R^n\to\zo$ is a degree-$d$ PTF with $\Ex_{\mun}[f] := \Delta \in \sbra{2^{-n}, 1-\epsilon}$.
In particular, suppose 
\[f(x) = \Indicator\{p(x) \geq \theta \}\]
where $p:\R^n\to\R$ is a degree-$d$ polynomial with $p(0) = 0$ and $\Var[p] = \sum_\alpha \wh{p}(\alpha)^2 = 1$. 
In this case, we have
\begin{equation} \label{eq:scaled-fourier-coeffs}
	\Ex_{\bx\sim\mun\upharpoonright_{f^{-1}(1)}}\sbra{\chi_\alpha(\bx)} = \frac{1}{\Delta}\Ex_{\bx\sim\mun}\sbra{f(\bx)\chi_\alpha(\bx)} = \frac{\wh{f}(\alpha)}{\Delta}.
\end{equation}

For any fixed pair $i,j$, by linearity of expectation we have
\begin{align*}
  \Ex_{\bx\sim\mun\upharpoonright_{f^{-1}(1)}}\sbra{ \bM } =
  & \Ex_{\bx\sim\mun\upharpoonright_{f^{-1}(1)}}\sbra{ \abra{ \tx{i}, \tx{j} } } \\ =
  & \abra{ \Ex_{\bx\sim\mun\upharpoonright_{f^{-1}(1)}}\sbra{ \tx{i} },
  \Ex_{\bx\sim\mun\upharpoonright_{f^{-1}(1)}}\sbra{ \tx{j} } } \\
  = & \norm{ \Ex_{\bx\sim\mun\upharpoonright_{f^{-1}(1)}}\sbra{ \tx{i} }}_2^2 \\
  = & \frac{1}{\Delta} \norm{ \Ex_{\bx\sim\mun}\sbra{ f(\bx) \tx{i} }}_2^2 \\
  = & \frac{1}{\Delta} \sum_{1\leq|S|\leq d} \wh{f}(S)^2 \\
  \geq & \frac{1}{\Delta}\cdot C_q(\mu)^{-\Theta(d)} \cdot \Delta^2.
\end{align*}

\begin{proposition}
  $\sum_{1\leq|S|\leq d} \wh{f}(S)^2 \geq C_q(\mu)^{-\Theta(d)} \Delta^2$.
\end{proposition}

\begin{proof}
  We want to prove
  \begin{align*}
    \sum_{1\leq |S|\leq d} \wh{f}(S)^2 \geq 2^{-\Theta(d)} \Ex_{\bx\sim\mun}\sbra{f(\bx)}^2.
  \end{align*}
  To that end, let us define another $\pm 1$ valued function
  $g(x) := \sign_{\pm 1} (f(x))$, and thus we have $g(x) = 2f(x) - 1$.
  As a result, for every non-empty $S$, $\wh{g}(S) = 2 \wh{f}(S)$.

  Also, by the anti-concentration we have for any $\theta^*$
  \begin{align*}
    \Ex_{\bx\sim\mun}\sbra{ |p(x) - \theta^*| } \geq C_q(\mu)^{-\Theta(d)}.
  \end{align*}
  Now using Cauchy-Schwarz, we have
  \begin{align*}
    \sqrt{ \left( \sum_{1\leq |S|\leq d} \wh{f}(S)^2 \right)
    \left( \sum_{1\leq |S|\leq d} \wh{p}(S)^2 \right) } \geq
    & \Ex_{\bx\sim\mun} \sbra{ f(\bx)\cdot p(\bx) } \\ =
    & \Ex_{\bx\sim\mun} \sbra{ 1_{p(\bx)\geq \theta} \cdot p(\bx) } \\ \geq
    & \theta \Ex_{\bx\sim\mun}\sbra{f(\bx)}.
  \end{align*}
  Since $\Var[p] = 1$, it follows that
  \begin{align*}
    \sum_{1\leq |S|\leq d} \wh{f}(S)^2 \geq \theta^2 \Ex_{\bx\sim\mun}\sbra{f(\bx)}^2.
  \end{align*}
  Then if $\theta \geq C_q(\mu)^{-\Theta(d)}$,
  we have our desired result.

  On the other hand, consider
  \begin{align*}
    \Ex_{\bx\sim\mun}\sbra{ g(\bx) (p(\bx) - \theta) } =
    \Ex_{\bx\sim\mun}\sbra{ |p(\bx) - \theta| } \geq C_q(\mu)^{-\Theta(d)},
  \end{align*}
  where the inequality follows from anti-concentration.
  This implies that
  \begin{align*}
    \sum_{1\leq |S|\leq d} \wh{g}(S) \wh{p}(S) - \theta \cdot \wh{g}(\emptyset) \geq C_q(\mu)^{-\Theta(d)}
  \end{align*}
  and thus
  \begin{align*}
    \sum_{1\leq |S|\leq d} \wh{g}(S) \wh{p}(S) \geq \theta \cdot \wh{g}(\emptyset) + C_q(\mu)^{-\Theta(d)}
  \end{align*}
  Then by Cauchy-Schwarz and $\wh{g}(S) = 2 \wh{f}(S)$ for any $S\neq \emptyset$, we get
  \begin{align*}
    \sum_{1\leq |S|\leq d} \wh{f}(S)^2 \geq \left( \theta \cdot \wh{g}(\emptyset) + C_q(\mu)^{-\Theta(d)} \right)^2
  \end{align*}
\end{proof}

\

\input{variance-truncates}

\
	
%\red{TODO: Final blurb once everything else is in place---Huan.}

\end{proofof}














==> sn-backup/variance-truncates.tex <==
Turning to the variance of the estimator, we have as before (cf. \Cref{eq:generic-variance}) that 
\[\Var[\bM] = {T\choose 2}^{-2}\pbra{\sum_{\substack{i<j\\k<l}} \Ex\sbra{\abra{\tx{i},\tx{j}}\abra{\tx{k},\tx{l}}} - \Ex\sbra{\abra{\tx{i},\tx{j}}}\Ex\sbra{\abra{\tx{k},\tx{l}}}}.\]
We once again have three cases:
\begin{enumerate}
\item When $|\cbra{i,j} \cap \cbra{k,l}| = 0$, then 
	\[\Ex\sbra{\abra{\tx{i},\tx{j}}\abra{\tx{k},\tx{l}}} - \Ex\sbra{\abra{\tx{i},\tx{j}}}\Ex\sbra{\abra{\tx{k},\tx{l}}} = 0.\]

\item When $|\cbra{i,j} \cap \cbra{k,l}| = 1$, because say $j = l$, then 
	\begin{align*}
		\Ex\sbra{\abra{\tx{i},\tx{j}}\abra{\tx{k},\tx{j}}} &\leq  \Ex\bigg[\pbra{\tx{i}}^T {\tx{j}\pbra{\tx{j}}^T}\tx{k}\bigg]\\
		&= \Ex\bigg[\pbra{\tx{i}}^T\bigg]\Ex\bigg[\underbrace{\tx{j}\pbra{\tx{j}}^T}_{=:V}\bigg]
\Ex\bigg[\tx{k}\bigg].
	\end{align*}
	One can check that $V$ is a $m\times m$ matrix whose $(\alpha_1, \alpha_2)^\text{th}$ entry (where $\alpha_1,\alpha_2 \in \N^n$ with $|\alpha_1|,|\alpha_2|\leq d$) is given by $\chi_{\alpha_1}(\x{j})\cdot\chi_{\alpha_2}(\x{j})$. 
	In particular, this lets us write
	\begin{align*}
	\Ex\sbra{\abra{\tx{i},\tx{j}}\abra{\tx{k},\tx{j}}} &= \sum_{|\alpha_1|,|\alpha_2|\leq d}\Ex\sbra{\chi_{\alpha_1}(\bx)}\Ex\sbra{\chi_{\alpha_1}(\by)\chi_{\alpha_2}(\by)}\Ex\sbra{\chi_{\alpha_2}(\bz)}\\
	&\leq \frac{1}{\Delta^2}\pbra{\sum_{|\alpha_1|,|\alpha_2|\leq d} \wh{f}(\alpha_1)^2\wh{f}(\alpha_2)^2}^{1/2}\pbra{{\sum_{|\alpha_1|,|\alpha_2|\leq d} \Ex\sbra{\chi_{\alpha_1}\chi_{\alpha_2}} ^2}}^{1/2}\\
%	&=\frac{\red{m}}{\Delta^3}\cdot O_d\pbra{\sum_{\substack{|\alpha_1|,|\alpha_2|\leq d \\ |\alpha_3|\leq 2d}} \wh{f}(\alpha_1)\wh{f}(\alpha_2)\wh{f}(\alpha_3)}\\
%	&\leq \frac{m}{\Delta^3}\cdot \pbra{\sum_{|\alpha_1|,|\alpha_2|\leq d} \wh{f}(\alpha_1)^2\wh{f}(\alpha_2)^2}^{1/2} O_d{\pbra{\sum_{|\alpha|\leq 2d} \wh{f}(\alpha)^2}^{1/2}}\\
%	&\leq \frac{m}{\Delta^2}\cdot O_d{\pbra{\sum_{|\alpha|\leq 2d} \wh{f}(\alpha)^2}^{1/2}}\\
	&\leq \frac{1}{\Delta}\pbra{{\sum_{|\alpha_1|,|\alpha_2|\leq d} \Ex\sbra{\chi_{\alpha_1}\chi_{\alpha_2}} ^2}}^{1/2}
	\end{align*}
	where the first inequality is by Cauchy-Schwarz and \Cref{eq:scaled-fourier-coeffs}, and the second is due to Parseval's formula.
	
\item When $|\cbra{i,j} \cap \cbra{k,l}| = 2$, then performing the same calculation as in the previous case gives that
	\begin{align*}
		\Ex\sbra{\abra{\tx{i},\tx{j}}\abra{\tx{i},\tx{j}}} &= \Ex\sbra{\pbra{\sum_{|\alpha|\leq d}\chi_\alpha\pbra{\x{i}}\chi_\alpha\pbra{\x{j}}}^2}\\
		&= \Ex\sbra{\sum_{|\alpha_1|,|\alpha_2|\leq d} \chi_{\alpha_1}\cdot\chi_{\alpha_2}\pbra{\x{i}}\chi_{\alpha_1}\cdot\chi_{\alpha_2}\pbra{\x{j}} } \\
		&= \sum_{|\alpha_1|,|\alpha_2|\leq d}	\Ex\sbra{\chi_{\alpha_1}\chi_{\alpha_2}}^2.
%&\leq\frac{m}{\Delta^2}\cdot O_d\pbra{\sum_{|\alpha|\leq 2d} \wh{f}(\alpha)^2}.
	\end{align*}
	
\end{enumerate}

We will now bound the final expressions obtained in the last two cases above. Note that \[\deg\pbra{\chi_{\alpha_1}\cdot\chi_{\alpha_2}} \leq 2d,\]
	and consequently $\chi_{\alpha_1}\cdot\chi_{\alpha_2} \in \mathrm{span}\pbra{\chi_\alpha}_{|\alpha|\leq 2d}$.  
	
\gray{	
	Note that when $\Delta \geq 2^{-d}$, we have by Parseval's formula that 
\[\sum_{|\alpha|\leq 2d}\wh{f}(\alpha)^2 \leq \sum_{\alpha}\wh{f}(\alpha)^2 = \Ex_{\mun}\sbra{f^2} = \Ex_{\mun}\sbra{f} = \Delta,\]
and so 
\[\Var[\bM] \leq {T\choose 2}^{-2}\cdot O_d\pbra{3{T\choose 3}\frac{m}{\Delta^{3/2}} + {T\choose 2}\frac{m}{\Delta}} \leq O_d\pbra{\frac{m}{T} + \frac{m}{T^2}}\]
as $\Delta \geq 2^{-d}$. 
}


